On the Feasibility of Multi-Mode Antennas in UWB and IoT Applications below 10 GHz

While on the one hand 5G and B5G networks are challenged by ultra-high data rates in wideband applications like 100+ Gbps wireless Internet access, on the other hand they are expected to support reliable low-latency Internet of Things (IoT) applications with ultra-high connectivity. These conflicting challenges are addressed in a system proposal dealing with both extremes. In contrast to most recent publications, focus is on the frequency domain below 10~GHz. Towards this goal, multi-mode antenna technology is used and different realizations, offering up to eight uncorrelated ports per radiator element, are studied. Possible baseband architectures tailored to multi-mode antennas are discussed, enabling different options regarding precoding and beamforming.

==> pic/Draw4Port6PortComparison.tex <==
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
		%\begin{semilogxaxis}[
		\begin{axis}[
		legend pos = north west ,
		legend columns = 1,
		legend style = {draw,fill=white},
		%xmode = log,
		%log basis x=10,
		legend cell align = left,
		width = 0.95\columnwidth,grid = both,
		%xmin = 0.9, xmax = 1.5e3, ymin = 0, ymax = 1e3,
		xmin = 0, xmax = 30, ymin = 0, ymax = 85,
		y tick label style={/pgf/number format/1000 sep=.},
		ylabel = Achievable sum-rate in ${{\textrm{bps}}/{\textrm{Hz}}}$,
		xlabel = Average user SNR in dB]
		
		\addplot[black, mark = o] table[x expr= \thisrow{TxSNR},y expr= \thisrow{rate_DS}, col sep = tab]{./pic/ict-sim-bb-US-F7.25-NUser10-NTeff726-mtx6-mrx1-Dist10-RUN100-NrfChains6-NFreq1_square16mm5.csv};
		\addplot[black, mark = x, dashed] table[x expr= \thisrow{TxSNR},y expr= \thisrow{rate_DS}, col sep = tab]{./pic/ict-sim-bb-US-F7.25-NUser10-NTeff484-mtx4-mrx1-Dist10-RUN100-NrfChains4-NFreq1_square4ports.csv};
		

	
		
		\addlegendentry{\small{6 ports per element}}
		\addlegendentry{\small{4 ports per element}}

		
		%\end{semilogxaxis}
		\end{axis}
	\end{tikzpicture}
	\caption{Sum-rate as a function of the average user SNR for digital beamforming with user scheduling, comparing the prototype antenna with four ports and the ideal square-shaped antenna providing six ports.}
	\label{fig: Draw4Port6PortComparison}
	
\end{figure}

==> pic/DrawCorrelationComparison.tex <==
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
		%\begin{semilogxaxis}[
		\begin{axis}[
		legend pos = north west,
		legend columns = 2,
		legend style = {draw,fill=white},
		%xmode = log,
		%log basis x=10,
		legend cell align = left,
		xtick = {-30,-27.5,...,-7.5},
		width = 0.95\columnwidth,grid = both,
		%xmin = 0.9, xmax = 1.5e3, ymin = 0, ymax = 1e3,
		%xmin = -30, xmax = -7.5, ymin = 0, ymax = 140,
		xmin = -15, xmax = -7.5, ymin = 0, ymax = 130,
		%y tick label style={/pgf/number format/1000 sep=.},
		ylabel = Achievable rate in bps/Hz,
		xlabel = Correlation between ports of a single element in dB]
		
		\addplot[black, every mark/.append style={solid}, mark = o] table[x expr= (\thisrow{Pxy}),y expr = \thisrow{dB20}, col sep = tab] {./pic/ict-sim-port-correlation-F7.25-NUser2-NTeff150-NReff6-mtx6-Dist10-RUN100-NrfChains8-NFreq1-mrx6.csv};
		\addplot[black, every mark/.append style={solid}, mark = o] table[x expr= (\thisrow{Pxy}),y expr = \thisrow{dB10}, col sep = tab]{./pic/ict-sim-port-correlation-F7.25-NUser2-NTeff150-NReff6-mtx6-Dist10-RUN100-NrfChains8-NFreq1-mrx6.csv};
		\addplot[black, every mark/.append style={solid}, mark = o] table[x expr= (\thisrow{Pxy}),y expr = \thisrow{dB0}, col sep = tab]{./pic/ict-sim-port-correlation-F7.25-NUser2-NTeff150-NReff6-mtx6-Dist10-RUN100-NrfChains8-NFreq1-mrx6.csv};
		
		\addplot[black,dashed, every mark/.append style={solid}, mark = x] table[x expr= (\thisrow{Pxy}),y expr = \thisrow{dB20}, col sep = tab]{./pic/ict-sim-port-correlation-F7.25-NUser2-NTeff100-NReff4-mtx4-Dist10-RUN100-NrfChains8-NFreq1-mrx4.csv};
		\addplot[black,dashed, every mark/.append style={solid}, mark = x] table[x expr= (\thisrow{Pxy}),y expr = \thisrow{dB10}, col sep = tab]{./pic/ict-sim-port-correlation-F7.25-NUser2-NTeff100-NReff4-mtx4-Dist10-RUN100-NrfChains8-NFreq1-mrx4.csv};
		\addplot[black,dashed, every mark/.append style={solid}, mark = x] table[x expr= (\thisrow{Pxy}),y expr = \thisrow{dB0}, col sep = tab]{./pic/ict-sim-port-correlation-F7.25-NUser2-NTeff100-NReff4-mtx4-Dist10-RUN100-NrfChains8-NFreq1-mrx4.csv};
	
		
		\addlegendentry{\small{6 ports}}
		\addlegendentry{\small{4 ports}}
		
		%\end{semilogxaxis}
		\end{axis}
	\end{tikzpicture}
	\caption{The expected achievable data rate as a function of correlation between the antenna ports of a single element. The assumptions are as follows: The BS has 25 elements, at two users receiver one antenna element is employed. A 150x12 (6 ports per element) and 100x8 (4 ports per element) massive MIMO system in downlink scenario is assumed. The channel is generated according to the WINNER II A1 NLOS scenario. A ZF precoding is employed for the analysis of the achievable rate.}
	\label{fig: DrawCorrelationComparison}
	
\end{figure}

==> pic/plots/Draw_CWC_NM4.tex <==

	\begin{tikzpicture}
		%\begin{semilogxaxis}[
		\begin{polaraxis}
		%xmin = 0,
		%xmax = 90,
		%xticklabel=$\pgfmathprintnumber{\tick}^\circ$,
		%xtick={0,30,...,330},
		%ytick={-10,-5,...,10},
	%	ymin=-10, ymax=10,
	%	axis line style={draw=none},
	%	axis tick style={draw=none},
		[
		xmin = -90,
		xmax = 90,
		width = 0.75\columnwidth,
		xticklabel=$\pgfmathprintnumber{\tick}^\circ$,
		xtick={120,150,...,330},
	%	ytick={-10,-5,...,10},
		ytick={15,20,...,30},
		%axis tick style={draw=none},
	%	ymin=-10, ymax=10,
		y coord trafo/.code=\pgfmathparse{#1+10},
		y coord inv trafo/.code=\pgfmathparse{#1-10},
	%	x dir=reverse,
		xticklabel style={anchor=-\tick-90,draw=none},
		yticklabel style={anchor=east, xshift=-1mm, yshift = -2.1mm,draw=none},
		legend style={at={(1.15,0.5)},nodes=left},
		legend columns = 6,
	%	ylabel = dBi,
		axis line style={draw=none},
		y label style={at={(axis description cs: -0.05,0.41)},rotate=0,draw=none},%,anchor=south},
		%	y axis line style={yshift=-4.75cm},
		%	ytick style={yshift=-4.75cm}
		]
	%	\addplot[no markers, thick, blue] table [col sep =comma, x index = {0},  y index = {1}] {./pic/E_NM4deg90.csv};
	%	\addplot[no markers, thick, green!80!black] table [col sep =comma, x index = {0},  y index = {2}] {./pic/E_NM4deg90.csv};
	%	\addplot[no markers, thick, red] table [col sep =comma, x index = {0},  y index = {3}] {./pic/E_NM4deg90.csv};
	%	\addplot[no markers, thick, black] table [col sep =comma, x index = {0},  y index = {4}] {./pic/E_NM4deg90.csv};
		
		\addplot[no markers, thick, blue] table [col sep =comma, x index = {0},  y index = {1}] {./CWC_4Modes_7.25_m10to10dB.csv};
		\addplot[no markers, thick, green!80!black] table [col sep =comma, x index = {0},  y index = {2}] {./CWC_4Modes_7.25_m10to10dB.csv};
		\addplot[no markers, thick, red] table [col sep =comma, x index = {0},  y index = {3}] {./CWC_4Modes_7.25_m10to10dB.csv};
		\addplot[no markers, thick, black] table [col sep =comma, x index = {0},  y index = {4}] {./CWC_4Modes_7.25_m10to10dB.csv};
		%\end{semilogxaxis}
	%	\legend{\footnotesize{Port 1}, \footnotesize{Port 2}, \footnotesize{Port 3}, \footnotesize{Port 4}}
		\end{polaraxis}
	\end{tikzpicture}


==> pic/plots/Draw_CWC_NM4__1_.tex <==

	\begin{tikzpicture}
		%\begin{semilogxaxis}[
		\begin{polaraxis}[
		width = 0.75\columnwidth,
		xticklabel=$\pgfmathprintnumber{\tick}^\circ$,
		xtick={0,30,...,330},
		ytick={-10,-5,...,10},
		ymin=-10, ymax=10,
		y coord trafo/.code=\pgfmathparse{#1+10},
		rotate=-90,
		y coord inv trafo/.code=\pgfmathparse{#1-10},
		x dir=reverse,
		xticklabel style={anchor=-\tick-90},
		yticklabel style={anchor=east, xshift=-1mm, yshift = -2.1mm},
		legend style={at={(1.15,0.5)},nodes=left},
		legend columns = 6,
		ylabel = dBi,
		y label style={at={(axis description cs: -0.05,0.41)},rotate=0},%,anchor=south},
	%	y axis line style={yshift=-4.75cm},
	%	ytick style={yshift=-4.75cm}
		]
	%	\addplot[no markers, thick, blue] table [col sep =comma, x index = {0},  y index = {1}] {./pic/E_NM4deg90.csv};
	%	\addplot[no markers, thick, green!80!black] table [col sep =comma, x index = {0},  y index = {2}] {./pic/E_NM4deg90.csv};
	%	\addplot[no markers, thick, red] table [col sep =comma, x index = {0},  y index = {3}] {./pic/E_NM4deg90.csv};
	%	\addplot[no markers, thick, black] table [col sep =comma, x index = {0},  y index = {4}] {./pic/E_NM4deg90.csv};
		
		\addplot[no markers, thick, blue] table [col sep =comma, x index = {0},  y index = {1}] {./pic/CWC_4Modes_7.25_m10to10dB.csv};
		\addplot[no markers, thick, green!80!black] table [col sep =comma, x index = {0},  y index = {2}] {./pic/CWC_4Modes_7.25_m10to10dB.csv};
		\addplot[no markers, thick, red] table [col sep =comma, x index = {0},  y index = {3}] {./pic/CWC_4Modes_7.25_m10to10dB.csv};
		\addplot[no markers, thick, black] table [col sep =comma, x index = {0},  y index = {4}] {./pic/CWC_4Modes_7.25_m10to10dB.csv};
		%\end{semilogxaxis}
		\legend{\footnotesize{Port 1}, \footnotesize{Port 2}, \footnotesize{Port 3}, \footnotesize{Port 4}}
		\end{polaraxis}
	\end{tikzpicture}

